Twenty-year monitoring of the surface magnetic fields of chemically peculiar stars

Magnetic chemically peculiar stars of the main sequence can present rotational periods as long as many decades. Here we report the results of an observational campaign started in 2001 aimed at establishing these very long periods from the variability of the integrated magnetic field modulus, the so-called surface magnetic field $B_s$, as measured from the Zeeman splitting of the Fe{\sc ii}\,6149.258\,{\AA} spectral line. Thirty-six stars have been monitored with various high-resolution spectrographs at different telescopes, totalling 412 newly collected spectra. To improve the phase coverage, we have also exploited all public archives containing high-resolution spectra, many not yet published. On the basis of these new $B_s$ variability curves, we 1) confirm or revisit the periods of 24 stars, 2) extend the lower limits to the periods of HD\,55719 ($P > 38$\,yr), HD\,165474 ($P > 27$\,yr), HD\,177765 ($P > 37$\,yr), 3) establish for the first time the periods of HD\,29578 ($P = 10.95$\,yr), HD\,47103 ($P = 17.683$\,d), HD\,150562 ($P = 5.7$\,yr), HD\,216018 ($P = 34.044$\,d), and 4) set lower limits to the periods of HD\,75445 ($P >> 14$\,yr), HD\,110066 ($P >> 29$\,yr), HD\,116114 ($P > 48$\,yr), and HD\,137949 ($P > 27$\,yr). As to $\gamma$\,Equ, whose period must exceed 90 years, we point out a clear decrease in the field modulus, the maximum of which coincides within the uncertainties with the minimum of the variation in the integrated longitudinal field.

==> HD137909_tab.tex <==
\begin{table}
\caption{Measured surface field of HD137909.}
\begin{tabular}{crrc|crrc}
HJD & B$_{\rm s}$ & err.& Sp & HJD & B$_{\rm s}$ & err.& Sp \\
2450000 & [G] & [G] & & 2450000 & [G] & [G]  \\ \hline
  2411.476 &  5392 &      100 & SG &   6816.429 &  5464 &       53 & CS \\ 
  3543.570 &  5474 &      100 & SG &   6816.437 &  5508 &       55 & CS \\ 
  3544.511 &  5663 &      100 & SG &   6816.488 &  5489 &       45 & CS \\ 
  3566.808 &  5590 &       40 & KE &   6820.469 &  5514 &       51 & CS \\ 
  3896.933 &  5576 &       40 & KE &   6820.484 &  5497 &       56 & CS \\ 
  6759.582 &  5446 &       52 & CS &   6820.500 &  5509 &       67 & CS \\ 
  6760.000 &  5413 &       51 & CS &   6822.422 &  5393 &       48 & CS \\ 
  6778.562 &  5456 &       47 & CS &   6822.429 &  5406 &       45 & CS \\ 
  6759.594 &  5395 &       46 & CS &   6822.402 &  5371 &       43 & CS \\ 
  6787.496 &  5453 &       45 & CS &   6826.410 &  5260 &       57 & CS \\ 
  6787.511 &  5413 &       37 & CS &   6826.418 &  5258 &       63 & CS \\ 
  6788.558 &  5478 &       57 & CS &   6826.379 &  5267 &       56 & CS \\ 
  6799.465 &  5761 &       64 & CS &   6828.398 &  5251 &       42 & CS \\ 
  6799.480 &  5687 &       45 & CS &   6830.469 &  5244 &       43 & CS \\ 
  6802.453 &  5687 &       52 & CS &   6830.472 &  5234 &       43 & CS \\ 
  6802.472 &  5564 &       52 & CS &   6830.511 &  5247 &       42 & CS \\ 
  6802.539 &  5532 &       55 & CS &   6831.418 &  5242 &       37 & CS \\ 
  6807.515 &  5366 &       48 & CS &   6831.394 &  5268 &       50 & CS \\ 
  6809.445 &  5369 &       53 & CS &   6844.359 &  5352 &       33 & CS \\ 
  6809.449 &  5385 &       55 & CS &   6844.367 &  5357 &       33 & CS \\ 
  6809.476 &  5298 &       40 & CS &   6848.332 &  5286 &       43 & CS \\ 
  6815.437 &  5392 &       57 & CS &   6848.379 &  5307 &       36 & CS \\ 
  6815.453 &  5419 &       57 & CS &   6849.336 &  5255 &       42 & CS \\ 
  6815.500 &  5421 &       55 & CS &   6849.344 &  5273 &       46 & CS \\ 
\hline
\end{tabular}
\end{table}


==> HD147010_tab.tex <==
\begin{table}
\caption{Measured surface field of HD147010.}
\begin{tabular}{crrc|crrc}
HJD & B$_{\rm s}$ & err.& Sp & HJD & B$_{\rm s}$ & err.& Sp \\
2450000 & [G] & [G] & & 2450000 & [G] & [G]  \\ \hline
  5411.793 & 11100 &      420 & ES &   4244.894 & 14600 &      300 & KE \\ 
  5412.742 & 14500 &      630 & ES &   6729.660 & 12150 &      300 & CS \\ 
  5414.738 & 11700 &      210 & ES &   6793.488 & 15200 &      300 & CS \\ 
  5961.094 & 12200 &      420 & ES &   6805.480 & 13800 &      300 & CS \\ 
  5967.113 & 13400 &      420 & ES &   6809.422 & 14200 &      300 & CS \\ 
  6099.961 & 15700 &      520 & ES &   6812.445 & 13350 &      300 & CS \\ 
  6100.859 & 12000 &      320 & ES &   6853.386 & 12350 &      300 & CS \\ 
  2826.742 & 12700 &      300 & KE &   7959.500 & 10000 &      300 & CS \\ 
\hline
\end{tabular}
\end{table}


==> HD59435_tab.tex <==
\begin{table}  \label{Tab_HD59435}
\scriptsize
\caption{Measured $B_s$ of HD59435.}
\begin{tabular}{ccc|ccc}
 \hline
 {HJD} & {B$_{\rm s}$} & {Sp} & {HJD} & {B$_{\rm s}$} & {Sp} \\
2400000+  & {[G]}                   &       &  {2400000+} & {[G]} &  ~\\\hline
53333.821 &  4300 $\pm$         100 & HS &54222.543 &  2380 $\pm$         100 & HS \\ 
53716.662 &  2510 $\pm$         100 & HS &56649.619 &  2470 $\pm$         100 & HN \\ 
 \hline
          \end{tabular} 
         \end{table}

